Vision-Language Model for Object Detection and Segmentation: A Review and Evaluation

Vision-Language Model (VLM) have gained widespread adoption in Open-Vocabulary (OV) object detection and segmentation tasks. Despite they have shown promise on OV-related tasks, their effectiveness in conventional vision tasks has thus far been unevaluated. In this work, we present the systematic review of VLM-based detection and segmentation, view VLM as the foundational model and conduct comprehensive evaluations across multiple downstream tasks for the first time: 1) The evaluation spans eight detection scenarios (closed-set detection, domain adaptation, crowded objects, etc.) and eight segmentation scenarios (few-shot, open-world, small object, etc.), revealing distinct performance advantages and limitations of various VLM architectures across tasks. 2) As for detection tasks, we evaluate VLMs under three finetuning granularities: \textit{zero prediction}, \textit{visual fine-tuning}, and \textit{text prompt}, and further analyze how different finetuning strategies impact performance under varied task. 3) Based on empirical findings, we provide in-depth analysis of the correlations between task characteristics, model architectures, and training methodologies, offering insights for future VLM design. 4) We believe that this work shall be valuable to the pattern recognition experts working in the fields of computer vision, multimodal learning, and vision foundation models by introducing them to the problem, and familiarizing them with the current status of the progress while providing promising directions for future research. A project associated with this review and evaluation has been created at https://github.com/better-chao/perceptual_abilities_evaluation.

==> tables/city2foggy.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Results (\%) on Cityscapes$ \rightarrow $Foggy Cityscapes.}
    \begin{tabular}{c|c|cccccccc|c|c}
        \hline
        Method & Finetuning Ways & person & rider & car & truck & bus & train & motor & bike & AP\textsubscript{50} & Reference \\
        \hline
        GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{12}{*}{Zero Prediction} &  &  &  &  &  &  &  &  &  & ECCV'24 \\
        GroundingDino (swin-L) ~\cite{liu2023grounding} &  &  &  &  &  &  &  &  &  &  & ECCV'24 \\
        GLIP-T (A) ~\cite{li2022grounded} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        GLIP-T (B) ~\cite{li2022grounded} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        GLIP-T (C) ~\cite{li2022grounded} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        RegionClip (Res50) ~\cite{zhong2022regionclip} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        RegionClip (Res50 $\times$ 4) ~\cite{zhong2022regionclip} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        OWL-ViT ~\cite{minderer2022simple} &  &  &  &  &  &  &  &  &  &  & Arxiv'22 \\
        OWLv2 ~\cite{minderer2024scaling} &  &  &  &  &  &  &  &  &  &  & NeurIPS'24 \\
        YOLO-World (Large) ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  & CVPR'24 \\
        YOLO-World (Mid) ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  & CVPR'24 \\
        PB-OVD ~\cite{gao2022open} &  &  &  &  &  &  &  &  &  &  & ECCV'22 \\
        \hline
        GroundingDino (swin-B)~\cite{liu2023grounding} & \multirow{6}{*}{Visual Finetuning} &  &  &  &  &  &  &  &  &  & ECCV'24 \\
        GLIP-T (A) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        GLIP-T (B) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        RegionClip (Res50) ~\cite{zhong2022regionclip} &  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        YOLO-World (Large) ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  & CVPR'24 \\
        PB-OVD ~\cite{gao2022open} &  &  &  &  &  &  &  &  &  &  & ECCV'22 \\
        \hline
        GroundingDino (swin-B)~\cite{liu2023grounding} & \multirow{5}{*}{Text Prompt} &  &  &  &  &  &  &  &  &  &  ECCV'24 \\
        GLIP-T (A) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        GLIP-T (B) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  & CVPR'22 \\
        YOLO-World (Large) ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  & CVPR'24 \\
        PB-OVD ~\cite{gao2022open} &  &  &  &  &  &  &  &  &  &  & ECCV'22 \\
        \hline
    \end{tabular}
\end{table*}


==> tables/det_dataset.tex <==
\begin{table*}[t]
    \centering
    \caption{Summary of the widely-used detection datasets for VLM evaluation.}
\begin{tabular}{l|rr|rr|rr|rr}
\toprule[1pt]
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{train} & \multicolumn{2}{c}{validation} & \multicolumn{2}{c}{trainval} & \multicolumn{2}{c}{test} \\
& images & objects& images   & objects   & images  & objects  & images& objects\\
\midrule
VOC~\cite{Pascal_VOC}~\href{http://host.robots.ox.ac.uk/pascal/VOC/voc2012/}{[link]} & 5717 & 13609 & 5823 & 13841 & 11540 & 27450 & 10991 & - \\
COCO~\cite{lin2014microsoft}~\href{http://cocodataset.org}{[link]} & 118287 & 860001 & 5000& 36781 & 123287 & 896782 & 40670 & - \\
LVIS~\cite{gupta2019lvis}~\href{http://www.lvisdataset.org}{[link]} & 100170 & 1270141 & 19809 & 244707 & 119979 & 1514848 & 19822 & - \\
Objects365~\cite{shao2019objects365}~\href{https://www.objects365.org/}{[link]} & 600000 & 9623000 & 38000 & 479000 & 638000 & 10102000 & 100000 & 170000 \\
OV-LVIS& 100170 & 1264884 & 4809 & 50672 & 104979 & 1315556 & - & - \\
OV-COCO& 107761 & 665387 & 4836 & 33152 & 112597 & 698539 & - & - \\
Stanford Dogs~\cite{khosla2011novel}~\href{http://vision.stanford.edu/aditya86/ImageNetDogs/}{[link]}& 12000 & 12000 & 8580 & 8580 & 20580 & 20580 & - & -  \\
CUB-200-2011~\cite{WahCUB_200_2011}~\href{https://www.vision.caltech.edu/datasets/cub_200_2011/}{[link]}& 5994 & 5994 & 5794 & 5794 & 11788 & 11788 & - & -  \\
Cityscapes~\cite{cordts2016cityscapes}~\href{https://www.cityscapes-dataset.com/}{[link]}& 2975 & 50347 & 500 & 9792 & 3475 & 60139 & 1525 & - \\
Foggy Cityscapes~\cite{sakaridis2018semantic}~\href{https://people.ee.ethz.ch/~csakarid/SFSU_synthetic/}{[link]}& 2975 & 50347 & 500 & 9792 & 3475 & 60139 & 1525 & -  \\
WaterColor~\cite{inoue2018cross}~\href{https://github.com/naoto0804/cross-domain-detection}{[link]}& 1000 & 1646 & - & - & 1000 & 1646 & 1000 & 1642  \\
Comic~\cite{inoue2018cross}~\href{https://github.com/naoto0804/cross-domain-detection}{[link]}& 1000 & 3164 & - & - & 1000 & 3164 & 1000 & 3138  \\
KITTI~\cite{geiger2012we}~\href{https://www.cvlibs.net/datasets/kitti/}{[link]}& - & - & - & - & 7481 & 28742 & 7518 & -  \\
Sim10K~\cite{johnson2016driving}~\href{https://fcav.engin.umich.edu/projects/driving-in-the-matrix}{[link]}& -& -& -& -& 10000 & 57776 & -& -  \\
ODinW~\cite{li2022grounded}~\href{https://huggingface.co/GLIPModel/GLIP}{[link]}& -& -& -& -& -& -& 20070& 135563 \\
VOC-C~\cite{michaelis2019benchmarking}~\href{https://github.com/bethgelab/robust-detection-benchmark}{[link]}& 543115& 1292855& 553185& 1314895& 1096300& 2607750& -& - \\
COCO-C~\cite{michaelis2019benchmarking}~\href{https://github.com/bethgelab/robust-detection-benchmark}{[link]}& 11237265& 81700095& 475000& 3494195& 11712265& 85194290& -& - \\
Cityscapes-C~\cite{michaelis2019benchmarking}~\href{https://github.com/bethgelab/robust-detection-benchmark}{[link]}& 282625& 4782965& 47500& 930240& 330125& 5713205& -& - \\
CrowdHuman~\cite{shao2018crowdhuman}~\href{https://www.crowdhuman.org/}{[link]}& 15000& 438792 & 4370 & 127716 & 19370 & 566508 & - & - \\
OCHuman~\cite{Zhang_2019_CVPR}~\href{https://github.com/liruilong940607/OCHumanApi}{[link]}& - & - & 2500 & 4291 & 2500 & 4291 & 2231 & 3819 \\
WiderPerson~\cite{zhang2019widerperson}~\href{http://www.cbsr.ia.ac.cn/users/sfzhang/WiderPerson/}{[link]}& 7891 & 244645 & 1000 & 28423 & 8891 & 273068 & 4382 & - \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/det_generalization_old.tex <==
\begin{table*}[htbp]

\centering
\caption{Open Vocabulary Generalization performance. For each setting, models are trained on the base categories of the dataset to the left of the arrow
 and tested on the full test set of the dataset to the right of the arrow.} 
\label{tab:det_generalization}
\resizebox{1.0\textwidth}{!}{%
    \begin{tabular}{l|l|ccc|ccc|ccc|ccc|l}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Fine-tuning Ways} & \multicolumn{3}{c|}{COCO$\rightarrow$ VOC} & \multicolumn{3}{c|}{COCO$\rightarrow$LVIS} & \multicolumn{3}{c|}{COCO$\rightarrow$Object365} & \multicolumn{3}{c|}{LVIS$\rightarrow$COCO}   & \multirow{2}{*}{Published} \\
\cline{3-14}          &  & AP$_{50}$ & AP$_{75}$ & AP    & AP$_{50}$ & AP$_{75}$ & AP & AP$_{50}$ & AP$_{75}$ & AP & AP$_{50}$ & AP$_{75}$ & AP  &  \\
    \midrule
    \midrule
    GroundingDino (swin-T) ~\cite{liu2023grounding} & \multirow{16}[2]{*}{Visual Fine-tuing} &81.6&71.2&64.9&29.4&25.1&23.5&33.1&27.4&25.1&65.6&54.3&49.5& ECCV’24 \\
    GLIP-T (A) ~\cite{li2022grounded} &       &    54.4   &    44.6   &    40.2   &  11.6   & 9.3 &  8.8  &   7.6  &  6.2  &  5.8 & 59.2  &    47.4   & 43.2 & CVPR’22 \\
    GLIP-T (B) ~\cite{li2022grounded} &       &    57.0   &     47.2  &   42.6  &  13.7   & 11.3 &   10.7   &   9.9 &  8.1  & 7.5    &     62.0  &    50.7   & 46.3 & CVPR’22 \\
    Region CLIP (Res50) ~\cite{zhong2022regionclip}  &       &    75.7   &   48.2  & 46.2 &  19.0   &   12.1   &    11.6   &   12.4   &    7.8    &    7.6  &    53.3   &   35.3    & 33.5 & CVPR’22 \\
    YOLO-World (Large) ~\cite{cheng2024yolo} &       &86.7       &74.8          &68.3    & 20.8&15.8      &   14.1    &30.4       &24.7       & 22.7      &52.9 &41.3       & 38.0      &CVPR’24 \\
    OVDINO (B) ~\cite{wang2024ov} &       &   83.2    &     71.8     & 65.3  &   52.3  &   44.0  &   41.4   &   36.3   &  29.5  &    27.2  & 63.0  &  52.7  & 47.9  & CVPR’24 \\
    PB-OVD ~\cite{gao2022open} &       &    59.3   &    36.1   &   34.9    &    6.5   &  3.7  &3.8&   7.7   &   4.7    & 4.6   &    41.8   &   24.2    & 23.9  & ECCV’22 \\
    OADP ~\cite{wang2023object} &       &    63.5   & 40.3      & 38.3       &  -     & -   & - &   -   &     -  &     - &  -     &    -   &- & ECCV'24 \\
    % BARON ~\cite{wu2023aligning} &       &    69.2   &    45.8   &    42.8   &       &    &&      &       &     &    -   &     -  & - & ECCV'24 \\
    BARON ~\cite{wu2023aligning} &       &    -   &    -   &    -  &    -   &  -  &-&    -  &    -   &   -  &    55.7  &     39.1  & 36.2 & CVPR'23 \\
    VL-PLM ~\cite{zhao2022exploiting}  &  & 46.3    &   69.7    &  50.3     &   3.1    &    2.3   &  2.1  &  7.5 &    5.4    &     5.0 &     -  &   -    &- & CVPR'22 \\
    % DST-Det ~\cite{xu2023dst} &       &         &       &       &       &    &&      &       &       & CVPR'22 \\
    Detic ~\cite{zhou2022detecting} &       &   62.1    &    40.2   &   38.1    &   10.9    &  7.6  & 7.1 &  6.8    &   4.6    &   4.3  &   57.7    &   38.7    &  36.2 &  CVPR'22 \\
    % OpenSeeD~\cite{zhang2023simple} &       &       &       &       &       &    &&      &       &    &       &       &   & Arxiv'22 \\
    PromptDet ~\cite{feng2022promptdet} &       &   -    &    -   &    -   &     -  &  -  &-&    -  &    -   & -   &  48.7     &    32.0   &  30.3 & CVPR'22 \\
    DetPro\cite{du2022learning}  &       &     -  &   -    &  -     &   -    &  -  &-&     - &   -    &   -  &   53.8   &      37.4  &34.9  & CVPR'22 \\
    % mm-ovod ~\cite{kaul2023multi}  &       &    -   &    -   &   -    &    -   &  -  &-&    -  &      - &  -   &       &       &  & NeurIPS'24 \\
    LAMI-DETR ~\cite{du2025lami} &       &   -    &  -     &   -    &    -   &  -  &-&  -    &  -     &  - &   57.6    &   46.9     &  42.8  & CVPR'24 \\
    \bottomrule
    % GroundingDino (swin-T) ~\cite{liu2023grounding} & \multirow{6}[2]{*}{Text Linear Probe} &  77.1   &67.7& 61.5     &27.1&21.9&20.2&       &       &    &       &       &   & ECCV’24 \\
    % GLIP-T (A) ~\cite{li2022grounded} &       &    75.7   &   63.3    &   57.2    &    19.5   &  15.5   & 14.8 &    0.6    &   0.6    &    0.6  &       &       & & CVPR’22 \\
    % GLIP-T (B) ~\cite{li2022grounded} &       &    80.1   &    68.3   &    61.9   &   18.2  & 14.7 &    13.9    &    1.2   &    1.1   &    1.1 &       &       &  & CVPR’22 \\
    % Region CLIP (Res50) ~\cite{zhong2022regionclip}  &       &   12.8     &   1.2  & 4.0 &   6.0  &    3.2   &   3.3    &   1.5    &   0.2    & 0.5  &       &       &    & CVPR’22 \\
    % YOLO-World (Large) ~\cite{cheng2024yolo} &       &       &          &    &&      &       &       &       &       & &       &       &CVPR’24 \\
    % OVDINO (B) ~\cite{wang2024ov} &       &   84.8    &     74.4     &  67.4  & 52.2 &  42.2    &    39.2   &    46.2   &    38.6   &  35.3  &       &       &   & CVPR’24 \\
    % PB-OVD ~\cite{gao2022open} &       &       &       &       &       &     &&     &       &    &       &       &   & ECCV’22 \\
    % \hline
    \end{tabular}%
}
\end{table*}


==> tables/det_semantic.tex <==
\begin{table*}[htbp]

\centering
\caption{Open Vocabulary recognition capability when ground truth bounding boxes are given, evaluated by Top-1 score. Models are trained on the coco base and test on the test set. } 
\label{tab:det_semantic}
\resizebox{1.0\textwidth}{!}{%
    \begin{tabular}{l|l|ccc|cccc|l}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Finetuning Ways} & \multicolumn{3}{c|}{COCO} & \multicolumn{4}{c|}{LVIS mini}     & \multirow{2}{*}{Published} \\
\cline{3-9}          &  & base & novel & all   & rare  & common & frequent & all   &  \\
    \hline
    GroundingDino(Tiny) ~\cite{liu2023grounding} & \multirow{6}[2]{*}{Zero Prediction} &  13.86     &   9.67    &  12.76     &    &  &  &       & ECCV’24 \\
    
    GLIP(A)  ~\cite{li2022grounded} &    &       &       &       &       &          &       &       & CVPR’22 \\
    Region CLIP(res50) ~\cite{zhong2022regionclip}  &       &       &          &       &       &       &       &       & CVPR’22 \\
    OVDINO(A)  ~\cite{wang2024ov}&       &       &          &       &       &       &       &       & Arxiv'24 \\
    YOLO-World(Large)  ~\cite{cheng2024yolo} &       & 15.01      &  10.39     &   13.80      &     &      &      &      & CVPR’24 \\
    PB-OVD ~\cite{gao2022open} &       &   5.40    &  5.97     &  5.55     &  0.00     &    0.21     &  1.88     &   1.30    & ECCV’22 \\
    \hline
    GroundingDino(Tiny) ~\cite{liu2023grounding} & \multirow{6}[2]{*}{Visual Finetuing} &   23.10    &    17.88   &  21.71     &    &  &  &       & ECCV’24 \\
    
    GLIP(A)  ~\cite{li2022grounded} &    &       &       &       &       &          &       &       & CVPR’22 \\
    Region CLIP(res50) ~\cite{zhong2022regionclip}  &       &       &          &       &       &       &       &       & CVPR’22 \\
    OVDINO(B) ~\cite{wang2024ov}&       &       &          &       &       &       &       &       & Arxiv'24 \\
    YOLO-World(Large)  ~\cite{cheng2024yolo} &       &   21.54    &  9.25     &    18.33     &     &      &      &      & CVPR’24 \\
    PB-OVD ~\cite{gao2022open} &       &  2.31     &  2.69     &  2.41     &  0.00     &    0.00     &  0.71     &   0.47    & ECCV’22 \\
    \hline
    % GroundingDino(Tiny) ~\cite{liu2023grounding} & \multirow{6}[2]{*}{Text Linear Probe} &       &       &       &    &  &  &       & ECCV’24 \\
    
    % GLIP(A)  ~\cite{li2022grounded} &    &       &       &       &       &          &       &       & CVPR’22 \\
    % Region CLIP(res50) ~\cite{zhong2022regionclip}  &       &       &          &       &       &       &       &       & CVPR’22 \\
    % OVDINO(B)  ~\cite{wang2024ov}&       &       &          &       &       &       &       &       & Arxiv'24 \\
    % YOLO-World(Large)  ~\cite{cheng2024yolo} &       &       &       &         &     &      &      &      & CVPR’24 \\
    % PB-OVD ~\cite{gao2022open} &       &  5.41     &   5.41    &    5.41   &   0.00    &    0.21     &   1.88    &  1.30     & ECCV’22 \\
    % \hline
    \end{tabular}%
}
\end{table*}


==> tables/domain_genelization_second.tex <==
\begin{table*}[htbp]
\centering
\caption{mAP comparison results for different weather conditions. For finetune, models are trained on the daytimeclear and test on the others dataset}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l|l|ccccc|l}
\hline
Method & Finetuning Ways & Day Clear & Night Clear & Dusk Rainy & Night Rainy & Day Foggy & Reference \\ \hline
OADP ~\cite{wang2023object} & \multirow{10}{*}{Visual finetuning} &  &  &  &  &  & ECCV'24 \\
BARON ~\cite{wu2023aligning} &  & &  &  &  &  & ECCV'24 \\
VL-PLM ~\cite{zhao2022exploiting} &  & &  &  &  &  & CVPR'22 \\
DST-Det ~\cite{xu2023dst}&  & &  &  &  &  & CVPR'22 \\
PromptDet ~\cite{feng2022promptdet}&  & &  &  &  &  & CVPR'22 \\
DetPro\cite{du2022learning} &  &  &  &  &  &  & CVPR'22 \\
Detic ~\cite{zhou2022detecting} &  & &  &  &  &  & CVPR'22 \\
OpenSeeD~\cite{zhang2023simple} &  & &  &  &  &  & Arxiv'22 \\
mm-ovod ~\cite{kaul2023multi} &  & &  &  &  &  & NeurIPS'24 \\
LAMI-DETR ~\cite{du2025lami}  &  &  &  &  &  &  & CVPR'24 \\
\hline
\end{tabular}
}
\end{table*}


==> tables/eva_gta5.tex <==
% !TEX root = ../main.tex
% !TEX spellcheck = en-US

% PREVIOUS VERSION OF TABLE IS BELOW

\begin{table*}[t]
  \centering
    \scalebox{0.73}{
    \begin{tabular}{cccccccccccccccccccc|c}
  \toprule
\rotatebox{90}{Method} & \rotatebox{90}{road} & \rotatebox{90}{sidewalk}& \rotatebox{90}{building} & \rotatebox{90}{wall}& \rotatebox{90}{fence} & \rotatebox{90}{pole}& \rotatebox{90}{light} & \rotatebox{90}{sign}& \rotatebox{90}{vegetation} & \rotatebox{90}{terrain}& \rotatebox{90}{sky} & \rotatebox{90}{person}& \rotatebox{90}{rider} & \rotatebox{90}{car}& \rotatebox{90}{truck} & \rotatebox{90}{bus}& \rotatebox{90}{train} & \rotatebox{90}{motocycle}& \rotatebox{90}{bicycle} & mIoU \\
  \midrule
  
CatSeg & 84.4& 18.7& 80.6& 23.8& 23.2& 28.4& 36.9& 23.4& 83.2& 25.2& {\bf 79.4}& 59.0& 29.9& 78.5& 33.7& 29.6& 1.7& {\bf 29.9}& 33.6& 42.30 \\
SAN  &  89.9 & 36.5 & 81.6 & {\bf 29.2} & 25.2 & 28.5 & 32.3 & 22.4 & {\bf 83.9} & 34.0 & 77.1 & 57.4 & 27.9 & 83.7 & 29.4 & 39.1 & 1.5 & 28.4 & 23.3 & 43.80   \\
SimpleBase  &  89.9 & 36.5 & 81.6 & {\bf 29.2} & 25.2 & 28.5 & 32.3 & 22.4 & {\bf 83.9} & 34.0 & 77.1 & 57.4 & 27.9 & 83.7 & 29.4 & 39.1 & 1.5 & 28.4 & 23.3 & 43.80   \\
MaskCLIP &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
DeOP &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
FC-CLIP &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
MAFT &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
SED &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
SCAN &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
OpenTrans &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\
EBSeg &  92.5 &  53.3 &  82.4& 26.5&  27.6& 36.4& 40.6& 38.9& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& 34.4& {\bf 84.9}&  34.1 & 53.1 & 16.9 & 27.7& 46.4 & 50.45 \\

  \bottomrule
  \end{tabular}
  }
  \caption{\small {\bf Results on GTA5$\rightarrow$CityScapes:} We evaluate on the $19$ common classes shared between these two dataset. Our method is consistently better compared to baselines, particularly for few number of labeled target domain images.}
  \label{tab:eva_gta5}
\end{table*}









% PREVIOUS VERSION OF THE TABLE
\iffalse

\begin{table*}
  \centering
    \scalebox{0.65}{
    \begin{tabular}{ccccccccccccccccccccc|c}
  \toprule
 \rotatebox{90}{\# City} & \rotatebox{90}{Method} & \rotatebox{90}{road} & \rotatebox{90}{sidewalk}& \rotatebox{90}{building} & \rotatebox{90}{wall}& \rotatebox{90}{fence} & \rotatebox{90}{pole}& \rotatebox{90}{light} & \rotatebox{90}{sign}& \rotatebox{90}{vegetation} & \rotatebox{90}{terrain}& \rotatebox{90}{sky} & \rotatebox{90}{person}& \rotatebox{90}{rider} & \rotatebox{90}{car}& \rotatebox{90}{truck} & \rotatebox{90}{bus}& \rotatebox{90}{train} & \rotatebox{90}{motocycle}& \rotatebox{90}{bicycle} & mIoU \\
  \midrule
    \multirow{3}{*}{\rotatebox{90}{0}} 
&MinEnt~\cite{Vu19} & 84.4& 18.7& 80.6& 23.8& 23.2& 28.4& 36.9& 23.4& 83.2& 25.2& {\bf 79.4}& 59.0& 29.9& 78.5& 33.7& 29.6& 1.7& {\bf 29.9}& 33.6& 42.3 \\
&AdvEnt~\cite{Vu19}  &  89.9 & 36.5 & 81.6 & {\bf 29.2} & 25.2 & 28.5 & 32.3 & 22.4 & {\bf 83.9} & 34.0 & 77.1 & 57.4 & 27.9 & 83.7 & 29.4 & 39.1 & 1.5 & 28.4 & 23.3 & 43.8   \\
&FDA-MBT~\cite{Yang20a} & {\bf 92.5}& {\bf 53.3}& {\bf 82.4}& 26.5& {\bf 27.6}& {\bf 36.4}& {\bf 40.6}& {\bf 38.9}& 82.3& {\bf 39.8}& 78.0& {\bf 62.6}& {\bf 34.4}& {\bf 84.9}& {\bf 34.1}& {\bf 53.1}& {\bf 16.9}& 27.7& {\bf 46.4}& {\bf 50.45}  \\
  \midrule
  \multirow{5}{*}{\rotatebox{90}{50}} 
&MinEnt~\cite{Vu19} & 92.56 & 56.84 &82.49 & 27.51 & 26.95 & 36.59 & 29.74 & 36.77 & 84.62 & 36.67 &78.21 & 60.54 &19.35 & 81.06 & 36.44 & 40.03 & 4.63 &19.36 & 52.34 & 47.51 \\
&AdvEnt~\cite{Vu19}  &  90.07 &  43.56 &  81.03 &  23.16 & 27.38 & 34.94 &27.52 &  28.04 & 84.6 & 26.59 & 75.73 & 60.9 &24.14 &  76.81 &39.09 &42.68 &  8.25 & 17.55 & 41.88 & 44.94   \\
&FDA-MBT~\cite{Yang20a} & 93.67& 59.62& 84.26&  {\bf 31.67}&  31.02&   36.99& 36.52&  42.06& 86.49&  {\bf 44.8}& 80.9&   {\bf 63.74}& {\bf 31.94}&  86.69& 47.16& 53.21 & {\bf 13.21} &33.84 & 50.39 & 53.06  \\
&ASS~\cite{Wang20} &  94.3 & 63.0 & 84.5 & 26.8 & 28.0 & 38.4 & 35.5 & 48.7 & {\bf 87.1} & 39.2& {\bf 88.8}& 62.2& 16.3& 87.6& 23.2& 39.2& 7.2& 24.4& {\bf 58.1}& 50.1    \\
&\ours{} & {\bf 94.39}&  {\bf 63.55} & {\bf 85.31} & 26.38 &{\bf 31.25} &{\bf 40.26} & {\bf 41.47} & {\bf 53.04} &87.08 & 43.38 &85.41 &62.88 & 30.11 & {\bf 87.9} &{\bf 48.33} & {\bf 55.22} & 8.34 & {\bf 34.01} &50.98 & {\bf 54.17}   \\
  \midrule
  \multirow{5}{*}{\rotatebox{90}{100}} 
&MinEnt~\cite{Vu19} & 92.98& 56.28& 83.15& 27.48& 25.9& 37.1 & 31.86 & 40.37 & 85.21 & 42.46 & 82.26&  60.62&  27.27&  83.7& 41.82& 45.32& 1.61& 20.9& 45.08& 49.02 \\
&AdvEnt~\cite{Vu19}  &  91.26&  51.02&   82.21&  23.18&  26.08& 37.25& 32.28&  33.01& 84.34&  34.25&   77.03&  61.72& 30.03&  84.04&  39.3& 42.27&  0.33& 16.17& 45.09& 46.89 \\
&FDA-MBT~\cite{Yang20a} &  94.43 &62.2 &85.21 &{\bf 32.74} &32.6 &38.58 &39.48 &47.6 &86.79 & 48.87 & 85.06 & 64.49 & 36.77 &  87.49 & 46.13 & {\bf 53.27} & 0.73 &32.98 & 52.44 & 54.1  \\
&ASS~\cite{Wang20} & {\bf 96.0}& {\bf 71.7}& 85.9& 27.9& 27.6& {\bf 42.8}& {\bf 44.7}& {\bf 55.9}& {\bf 87.7}& 46.9& {\bf 89.0}& {\bf 66.0}& 36.4& 88.4& 28.9& 21.4& {\bf 11.4}& 38.0& {\bf 63.2}& 54.2   \\
&\ours{} & 94.6 &  66.06 &  {\bf 86.25} &  26.17 & {\bf 34.93} &  38.89 & 40.48 &  52.93 & 87.26 & {\bf 49.2} &  87.89 &64.7 &  {\bf 36.77} & {\bf 88.6} & {\bf 48.39} &  45.04 & 2.77 & {\bf 38.8} &  58.49 & {\bf 55.17}   \\
  \midrule
  \multirow{5}{*}{\rotatebox{90}{200}} 
&MinEnt~\cite{Vu19} & 93.94& 59.01&  84.69& 22.4& 30.21& 38.35& 36.18& 47.3& 86.02& 42.38& 82.36& 62.08& 32.98& 87.08& 44.24&  38.96& {\bf 28.49}& 20.32& 52.3& 52.07 \\
&AdvEnt~\cite{Vu19}  & 92.71&   58.38&  84.04&  22.36& 30.13 &  36.31 & 37.33&  43.4 & 85.6 & 35.73 &  83.42 & 61.34 &  27.95 &  80.91 & 39.49 &41.62 & 22.9 & 19.01 &  51.69 & 50.23   \\
&FDA-MBT~\cite{Yang20a} &   94.68 &62.76 & 85.87 &  {\bf 32.92} &  31.94 &  38.49 &  41.93 &  51.66 & 86.88 & 47.48 & 85.15 & 64.78 &  36.72 & 87.93 & {\bf 48.63} & {\bf 58.22} & 19.17 & 37.01 & 54.89 & 56.16   \\
&ASS~\cite{Wang20} & {\bf 96.1}& {\bf 71.9}& 85.8& 28.4& 29.8& {\bf 42.5}& 45.0& {\bf 56.2}& {\bf 87.4}& 45.0& {\bf 88.7}& 65.8& 38.2& {\bf 89.6}& 42.2& 35.9& 17.1& 35.8& {\bf 61.6}& 56.0    \\
&\ours{} &  94.17 & 62.23& {\bf 85.91} & 29.01& {\bf 34.95}&  41.74&{\bf 45.74}& 55.41&87.36& {\bf 49.05}& 86.09 & {\bf 65.82} & {\bf 40.2} &  88.77& 47.58& 58.07&12.72& {\bf 40.19}& 57.17 & {\bf 56.96}  \\
  \midrule
  \multirow{5}{*}{\rotatebox{90}{500}} 
&MinEnt~\cite{Vu19} & 94.76 & 65.6 & 85.99 & 32.07 & 37.27 & 40.7 & 40.45 & 53.69 &  86.72 &  44.77 &  86.26 & 63.22 & 31.01 &  86.31 & 49.77 & 53.59 &  13.08 &  26.68 &  58.1 &  55.26 \\
&AdvEnt~\cite{Vu19}  & 94.94 &  67.53 &  85.65 & 28.42 & 36.3 &41.25 & 40.8 &  53.14 & 87.32 & 45.6 & 84.35 & 64.23 & 36.4 & 87.47 & 50.67 & 46.87 & 13.41 & 29.2 & 59.4 & 55.42   \\
&FDA-MBT~\cite{Yang20a} &  94.61 &  64.93 &  86.64 & {\bf 36.33} &   38.9 &  42.59 &  46.23 &  56.37 & 87.82 &  {\bf 52.35} &   85.85 & 65.93 &    39.37 &  89.28 &  56.41 &    61.96 &  {\bf 23.56} &  39.3 &  56.1 & 59.19   \\
&ASS~\cite{Wang20} & {\bf 96.2}& {\bf 72.7}& {\bf 87.6}& 35.1& 31.7& {\bf 46.6}& 46.9& {\bf 62.7}& {\bf 88.7}& 49.6& {\bf 90.5}& {\bf 69.2}& 42.7& {\bf 91.1}& 52.6& 60.9& 9.6& {\bf 43.1}& {\bf 65.6}& 60.2   \\
&\ours{} & 94.67 & 66.73 & 87.43 & 31.5 &{\bf 42.47} &42.18 & {\bf 46.97} & 58.45 &87.72 & 49.68 & 88.51 &68.07 &{\bf 44.49} &  89.5 & {\bf 62.32} &  {\bf 62.08} & 19.69 &  42.56 &   63.17 & {\bf 60.43}   \\
  \midrule
  \multirow{5}{*}{\rotatebox{90}{1000}} 
&MinEnt~\cite{Vu19} &  95.53 &  70.35 &   86.74 & 33.3 & 35.65 &  41.64 &  44.4 &  55.94 &  87.3 &  46.11 &  87.52 & 64.79 & 38.29 & 88.19 & 45.77 & 59.4 & 34.0 & 33.96 & 60.62 & 58.4 \\
&AdvEnt~\cite{Vu19}  &  95.43 & 70.13& 86.32& 35.88& 38.74& 40.52& 43.72&  55.44& 87.74& 50.54& 87.13& 65.56&  40.62&  87.9& 56.89& 50.98&  10.27&  36.74&  61.14&  57.98   \\
&FDA-MBT~\cite{Yang20a} & 95.98 & 71.85 &  87.16 & 31.7 & 39.73 & 43.97 & 47.52 & 59.09 & 88.02 & 51.13 &     88.78 &  69.35 &  47.78 &  89.93 & 62.96 & 67.17 & 36.6 & 45.94 &  60.29 &62.37  \\
&ASS~\cite{Wang20} & {\bf 96.8}& {\bf 76.3}& {\bf 88.5}& 30.5& 41.7& {\bf 46.5}& 51.3& {\bf 64.3}& {\bf 89.1}& {\bf 54.2}& {\bf 91.0}& 70.7& 48.7& {\bf 91.6}& 59.9& 68.0& {\bf 40.8}& {\bf 48.0}& {\bf 67.0}& 64.5   \\
&\ours{} &  96.09 & 72.45 &  88.47 & {\bf 38.9} &  {\bf 47.68} &  45.76 &  {\bf 51.57} &   61.66 & 88.86 &   50.89 &   89.06 &  {\bf 71.43} &  {\bf 51.01} &   91.31 &  {\bf 68.11} &  {\bf 69.42} &  32.53 &  46.21 & 66.4 & {\bf 64.62}    \\
  \bottomrule
  \end{tabular}
  }
  \caption{ {\bf Quantitative Comparison on GTA5$\rightarrow$CityScapes.} We evaluate on the $19$ common classes shared between these two dataset. Note that our method consistently achieves better performance than the others across different number of labelled target domain images. }
  \label{tab:eva_gta5}
\end{table*}

\fi

==> tables/mess_table.tex <==
\begin{table*}[!t]
    \begin{center}
    
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{l|ccccc|c}
\toprule

Model & General & Earth Monit. & Medical Sciences & Engineering & Agri. and Biology & Mean \\
\midrule
% \textit{Random (LB)} & - & - & \phantom{0}\textit{1.17} & \phantom{0}\textit{7.11} & \textit{29.51} & \textit{11.71} & \phantom{0}\textit{6.14} & \textit{10.27} \\
% \textit{Best supervised (UB)} & - & - & \textit{48.62} & \textit{79.12} & \textit{89.49} & \textit{67.66} & \textit{81.94} & \textit{70.99} \\
% \midrule
Cat-Seg~\cite{cho2024cat} & & & & & & \\
SAN~\cite{xu2023side}  & \underline{29.35} & \underline{30.64} & 29.85 & \textbf{23.58} & 15.07 & \underline{26.74} \\
SimpleBase~\cite{xu2022simple}  & 19.98 & 17.98 & \underline{41.82} & 14.0\phantom{0} & 22.32 & 22.73 \\
ZegFormer~\cite{ding2022decoupling}  & 13.57 & 17.25 & 17.47 & 17.92 & \underline{25.78} & 17.57 \\
ZegCLIP~\cite{zhou2023zegclip} & & & & & & \\ 
MaskCLIP~\cite{ding2022open} & & & & & & \\ 
DeOP~\cite{han2023open} & & & & & & \\ 
FC-CLIP~\cite{yu2024convolutions} & & & & & & \\ 
MAFT~\cite{jiao2023learning} & & & & & & \\ 
SED~\cite{xie2024sed} & & & 35.37 & 21.91 & 35.01 &\\
SCAN~\cite{liu2024open} & & & & & & \\
OpenTrans~\cite{xu2024transferable} & & & & & & \\ 
EBSeg~\cite{shan2024open} & & & & & & \\ 
SegCLIP~\cite{luo2023segclip} & & & & & & \\ 
TCL~\cite{cha2023learning} & & & & & & \\
MaskCLIP~\cite{zhou2022extract} & & & & & & \\ 
CLIPtrase~\cite{shao2024explore} & & & & & & \\ 
% X-Decoder~\cite{zou2023generalized} & 22.01 & 18.92 & 23.28 & 15.31 & 18.17 & 19.8\phantom{0} \\
% OpenSeeD~\cite{zhang2023simple} & 22.49 & 25.11 & \textbf{44.44} & 16.5\phantom{0} & 10.35 & 24.33 \\
% \hlrow & & & \textbf{38.69} & \textbf{35.91} & 28.09 & \underline{20.34} & \textbf{32.57} & \textbf{31.96} \\
% \hlrow\multirow{-2}{*}{\ours (ours)} & \multirow{-2}{*}{CLIP ViT-B/16} & \multirow{-2}{*}{-} & \textcolor{ForestGreen}{(+9.34)} & \textcolor{ForestGreen}{(+5.27)} & \color{gray}{(-16.35)} & \color{gray}{(-3.24)} & \textcolor{ForestGreen}{(+6.79)} & \textcolor{ForestGreen}{(+5.22)} \\
% \midrule
% OVSeg~\citep{liang2022open} & CLIP ViT-L/14 & Swin-B & 29.54 & 29.04 & \textbf{31.9\phantom{0}} & 14.16 & \underline{28.64} & 26.94 \\
% SAN~\citep{xu2023side} & CLIP ViT-L/14 & - & \underline{36.18} & \underline{38.83} & \underline{30.27} & \underline{16.95} & 20.41 & \underline{30.06} \\
% \hlrow & & & \textbf{44.69} & \textbf{39.99} & 24.70 & \textbf{20.20} & \textbf{38.61} & \textbf{34.70} \\
% \hlrow\multirow{-2}{*}{\ours (ours)} & \multirow{-2}{*}{CLIP ViT-L/14} & \multirow{-2}{*}{-} & \textcolor{ForestGreen}{(+8.51)} & \textcolor{ForestGreen}{(+1.16)} & \color{gray}{(-7.2)} & \textcolor{ForestGreen}{(+3.25)} & \textcolor{ForestGreen}{(+9.97)} & \textcolor{ForestGreen}{(+4.64)} \\
% & 44.49 & 22.40 & 5.09 & 6.96 & 27.3 & 19.03 & 3.7 & 33.87  & 36.67 & 24.19 & 38.15
% 
% 
        \bottomrule
    \end{tabular}
    }
    \vspace{-5pt}        
    \caption{\textbf{Quantitative evaluation on MESS.} }
    \label{tab:mess_}
    \vspace{-20pt}
    \end{center}
\end{table*}


==> tables/ovd_second_model_continued_summary.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Summary of the Second Type of Open Vocabulary Detection Models(Continued)}
    \begin{tabular}{p{2cm}|p{3cm}|p{1.8cm}|p{3cm}|p{4cm}|p{1.5cm}}
        \hline
        Method & Image Encoder & Text Encoder & Datasets & Contribution & Published \\
        \hline
        % Detic\cite{zhou2022detecting} \href{https://github.com/facebookresearch/Detic}{[code]} & CenterNet2 (ResNet50) & CLIP-text & LVIS-base, IN-L (997 overlapping IN-21K classes with LVIS), CC & Propose training detector classifiers on image classification data to enable detection of a wide range of concepts. & ECCV 2022 \\
        % VLDet\cite{lin2022learning} \href{https://github.com/clin1223/VLDet}{[code]} & \makecell[l]{1. Faster RCNN(ResNet50) \\ 2. CenterNet2(ResNet50)} & CLIP-text & \makecell[l]{1. COCO-base, \\COCO Caption \\ 2. LVIS-base, \\Conceptual Captions} & Learn from image-text pairs by formulating object-language alignment as a set matching problem between image region features and word embeddings. & ICLR 2023 \\
        % DetPro\cite{du2022learning} \href{https://github.com/dyabel/detpro}{[code]} & Faster RCNN(ResNet50) & CLIP-text & LVIS-base & Propose a novel method for learning continuous prompt representations for open-vocabulary object detection. & CVPR 2022 \\
        % OV-DETR\cite{zang2022open} \href{https://github.com/yuhangzang/OV-DETR}{[code]} & Deformable DETR(ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose an open-vocabulary detector based on DETR, enabling object detection from class names or exemplar images by formulating the task as a binary matching problem using CLIP. & ECCV 2022 \\
        % ViLD\cite{gu2021open} \href{https://github.com/tensorflow/tpu/tree/master/models/official/detection/projects/vild}{[code]} & Mask RCNN(ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose to distill knowledge from a pre-trained VLM into a two-stage object detector by aligning the student's region embeddings with the teacher's text and image embeddings. & ICLR 2022 \\
        % HierKD\cite{ma2022open} \href{https://github.com/mengqiDyangge/HierKD}{[code]} & ATSS(ResNet50) & CLIP-text & COCO-base & Propose a hierarchical visual-language knowledge distillation method for open-vocabulary one-stage detectors, combining global and instance-level distillation. &  CVPR 2022 \\
        % PromptDet\cite{feng2022promptdet} \href{https://github.com/fcjian/PromptDet}{[code]} & Mask RCNN(ResNet50) & CLIP-text & LVIS-base, LAION-novel & Propose regional prompt learning to align textual embeddings with visual object features and a self-training framework to scale detection without manual annotations. & ECCV 2022 \\
        % BARON\cite{wu2023aligning} \href{https://github.com/wusize/ovdet}{[code]} & Faster RCNN(ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose a method to enhance open-vocabulary object detection by aligning the embedding of a bag of regions. & CVPR 2023 \\
        % CoDet\cite{ma2024codet} \href{https://github.com/CVMI-Lab/CoDet}{[code]} & \makecell[l]{1. Faster R-CNN(ResNet50) \\ 2. CenterNet2(ResNet50)} & CLIP-text & \makecell[l]{1. COCO-base,\\ COCO Caption \\ 2. LVIS-base, CC3M} & Reformulate region-word alignment as a co-occurring object discovery problem, leveraging visual similarities to discover and align objects with shared concepts mentioned in grouped image captions. & NeurIPS 2023 \\
        % CORA\cite{wu2023cora} \href{https://github.com/tgxs002/CORA}{[code]} & DAB DETR(CLIP-ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose a DETR-style framework that adapts CLIP using Region prompting to address the whole-to-region distribution gap and Anchor pre-matching for improved object localization. & CVPR 2023 \\
        % DK-DETR\cite{li2023distilling} \href{https://github.com/hikvision-research/opera/tree/main/configs/dk-detr}{[code]} & Deformable DETR(ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose a framework that distills semantic and relational knowledge from VLM into a DETR-like detector & ICCV 2023 \\
        % DST-Det\cite{xu2023dst} \href{https://github.com/xushilin1/dst-det}{[code]} & Mask RCNN (ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base \\ 3. V3-Det-base} & Propose a strategy that leverages the zero-shot classification ability of pre-trained VLM to generate pseudo-labels for novel classes. & Preprint \\
        % EdaDet\cite{shi2023edadet} & DETR(ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose Early Dense Alignment (EDA) to improve base-to-novel generalization by learning dense-level alignment with object-level supervision. & ICCV 2023 \\
        F-VLM\cite{kuo2022f} \href{https://github.com/google-research/google-research/tree/master/fvlm}{[code]} & Mask RCNN (CLIP-ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Simplify training by using a frozen vision-language model and fine-tuning only the detector head. & ICLR 2023 \\
        MM-OVOD\cite{kaul2023multi} \href{https://github.com/prannaykaul/mm-ovod}{[code]} & CenterNet2 (ResNet50) & CLIP-text & LVIS-base, IN-L (997 overlapping IN-21K classes with LVIS) & Propose generating text-based classifiers with a large language model, employing a visual aggregator for image exemplars, and fusing both to create a multi-modal classifier, introducing a novel approach for ovod. & ICML 2023 \\
        OADP\cite{wang2023object} \href{https://github.com/LutingWang/OADP}{[code]} & Faster RCNN (ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose an Object-Aware Knowledge Extraction module for precise object knowledge extraction and a Distillation Pyramid mechanism for comprehensive global and block distillation. & CVPR 2023 \\
        Prompt-OVD\cite{song2023prompt} & Deformable DETR (ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose to use CLIP class embeddings as prompts, along with RoI-based masked attention and RoI pruning to enhance detection performance with minimal computational cost. & Preprint \\
        RO-ViT\cite{kim2023region} \href{https://github.com/google-research/google-research/tree/master/fvlm/rovit}{[code]} & Mask RCNN (Pretrained ViT) & Transformer & \makecell[l]{Pretraining: ALIGN \\ 1. COCO-base \\ 2. LVIS-base} & Propose randomly cropping and resizing regions of positional embeddings to align with region-level detection, replacing softmax cross entropy with focal loss for better handling difficult examples. & CVPR 2023 \\
        SAS-Det\cite{zhao2024taming} \href{https://github.com/xiaofeng94/SAS-Det}{[code]} & Faster RCNN (CLIP-ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Propose a split-and-fusion head to separate open and closed branches for complementary learning and reduces noisy supervision, along with a periodic update strategy to stabilize pseudo-label distributions. & CVPR 2024 \\
        CLIPSELF\cite{wu2023clipself} \href{https://github.com/wusize/CLIPSelf}{[code]} & Mask RCNN (finetuned CLIP-ViT) & CLIP-text & \makecell[l]{1. COCO base \\ 2. LVIS base} & Adapt CLIP ViT's image-level recognition to local regions by self-distilling region representations from its dense feature map. & ICLR 2024 \\
        LP-OVOD\cite{pham2024lp} \href{https://github.com/VinAIResearch/LP-OVOD}{[code]} & Faster RCNN (ResNet50) & CLIP-text & \makecell[l]{1. COCO-base \\ 2. LVIS-base} & Discard low-quality boxes by training a sigmoid linear classifier on pseudo labels retrieved from the top relevant region proposals to the novel text. & WACV 2024 \\
        \hline
    \end{tabular}
\end{table*}



==> tables/seg_datasets.tex <==
\begin{table*}[t]
    \centering
    \caption{Summary of the widely-used visual recognition datasets for VLM evaluation. \textcolor{magenta}{[link]} directs to dataset websites.}
    \label{tab.eval_datasets}
    \begin{tabular}{l|c|c|c|c|c}
        \toprule[1pt]
        \textbf{Dataset} & \textbf{Year} &\textbf{Classes} & \textbf{Training} & \textbf{Testing} & \textbf{Evaluation Metric} \\
        \midrule
        COCO-Stuff~\cite{}~\href{https://github.com/nightrome/cocostuff}{[link]} & 2018&172&118k&20k&mIoU\\
        PASCAL VOC 2012~\cite{everingham2010pascal}~\href{http://host.robots.ox.ac.uk/pascal/VOC/voc2012/}{[link]} & 2012 & 20 & 1464 & 1449 & mIoU\\
        PASCAL Content~\cite{mottaghi2014role}~\href{https://www.cs.stanford.edu/~roozbeh/pascal-context/}{[link]} & 2014 &459&4998&5105 &mIoU\\
        Cityscapes~\cite{cordts2016cityscapes}~\href{https://www.cityscapes-dataset.com/}{[link]}& 2016 &19&2975&500&mIoU \\
        ADE20k~\cite{zhou2017scene}~\href{https://groups.csail.mit.edu/vision/datasets/ADE20K/}{[link]}&2017&150& 25574 & 2000 & mIoU \\
        MESS*~\cite{}~\href{https://github.com/blumenstiel/MESS}{[link]}& 2023 & - & - & - & mIoU \\
        FSS-1000~\cite{}~\href{https://github.com/HKUSTCV/FSS-1000}{[link]} & 2020 & 1000 & 5200 & 2400 & mIoU \\
        PASCAL-Part~\cite{}~\href{https://roozbehm.info/pascal-parts/pascal-parts.html}{[link]} & 2020 & 17 & 8432 & 851 & mIoU \\
        ADE20k-part~\cite{}~\href{}{[link]} & 2008 & 44 & 7348 & 1017 & mIoU \\
        CamVid~\cite{}~\href{https://mi.eng.cam.ac.uk/research/projects/VideoRec/CamVid/}{[link]}&2008&11& 467 & 233 & mIoU \\
        UAVid~\cite{}~\href{https://uavid.nl/}{[link]}& 2018 & 9 & 200 & 100 & mIoU \\
        UDD6~\cite{}~\href{https://github.com/MarcWong/UDD}{[link]}& 2018 & 12 & 205 & 45 & mIoU \\
        \bottomrule[1pt]
    \end{tabular}
    
\end{table*}

==> tables/three_adaptation_second.tex <==
\begin{table*}[htbp]
\centering
\caption{For finetune, models are trained on the dataset on the left of the arrow and test on the dataset on the right of the arrow.} 
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|c|c|c|c|c}
\hline
\multirow{2}{*}{Method}& \multirow{2}{*}{Finetuning Ways}& {Cityscapes→FoggyCityscapes}& {Sim10K→Cityscapes} &  {KITTI→Cityscapes} &  {Cityscapes→KITTI}  &  \multirow{2}{*}{Reference} \\ \cline{3-6}
 & & AP$_{50}$  & AP$_{50}$ & AP$_{50}$    & AP$_{50}$    &  \\ \hline
OADP ~\cite{wang2023object} &  \multirow{10}{*}{Visual finetuning}  & & & & &  ECCV'24 \\
BARON ~\cite{wu2023aligning} &  &  & &  & &  ECCV'24 \\
VL-PLM ~\cite{zhao2022exploiting}   &   & & & &  &  CVPR'22 \\
DST-Det ~\cite{xu2023dst}   &   & & & &  &  CVPR'22 \\
PromptDet ~\cite{feng2022promptdet}   &  &  & & &  &  CVPR'22 \\
DetPro\cite{du2022learning}  &  &  &  &  &  &  CVPR'22 \\
Detic ~\cite{zhou2022detecting}   &  &  & & &  &  CVPR'22 \\
OpenSeeD~\cite{zhang2023simple}  &  &  & & &  &  Arxiv'22 \\
mm-ovod ~\cite{kaul2023multi}   &  & & & &   &  NeurIPS'24 \\
LAMI-DETR ~\cite{du2025lami} & &  &  &  & &   CVPR'24 \\
\hline
\end{tabular}
}
\end{table*}


==> tables/three_adaptions.tex <==
\begin{table*}[htbp]
\centering
\caption{For finetune, models are trained on the dataset on the left of the arrow and test on the dataset on the right of the arrow.} 
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|c|c|c|c|c}
\hline
\multirow{2}{*}{Method}& \multirow{2}{*}{Finetuning Ways}& {Cityscapes→FoggyCityscapes}& {Sim10K→Cityscapes} &  {KITTI→Cityscapes} &  {Cityscapes→KITTI}  &  \multirow{2}{*}{Reference} \\ \cline{3-6}
 & & AP$_{50}$  & AP$_{50}$ & AP$_{50}$    & AP$_{50}$    &  \\ \hline
GroundingDino (swin-T) ~\cite{liu2023grounding} &  \multirow{12}{*}{Zero Prediction}  & 34.4 & 45.0 &45.0 & 80.0&  ECCV'24 \\
GroundingDino (swin-B) ~\cite{liu2023grounding} &  &42.4  &52.0 & 52.0 &74.9 &  ECCV'24 \\
GLIP-T (A) ~\cite{li2022grounded}   &   & 31.8& 44.3& 44.3& 82.3 &  CVPR'22 \\
GLIP-T (B) ~\cite{li2022grounded}   &   &27.4 &37.8 &37.8 & 80.6 &  CVPR'22 \\
GLIP-T (C) ~\cite{li2022grounded}   &  & 29.6 &40.6 & 40.6& 81.2 &  CVPR'22 \\
RegionClip (Res50) ~\cite{zhong2022regionclip}  &  & 13.5 & 36.3 & 36.3 & 7.09 &  CVPR'22 \\
RegionClip (Res50 $\times$ 4) ~\cite{zhong2022regionclip}   &  &  14.3& 36.3& 36.3&  53.7&  CVPR'22 \\
OVDINO (A) ~\cite{wang2024ov}  &  & 36.6 &76.4 & 76.4& 67.7 &  Arxiv'22 \\
OVDINO (B) ~\cite{wang2024ov}   &  & 40.7 &76.6 & 76.6& 71.5 &  NeurIPS'24 \\
YOLO-World (Large) ~\cite{cheng2024yolo}  & & 28.9 & 40.6 & 40.6 & 79.7&   CVPR'24 \\
YOLO-World (Mid) ~\cite{cheng2024yolo}   & &25.8  &36.1 &36.1 &78.1   &   CVPR'24 \\
PB-OVD ~\cite{gao2022open}   &   &9.8 &13.3  & 13.3 & 39.9  & ECCV'22 \\
\hline
GroundingDino (swin-T) ~\cite{liu2023grounding} &  \multirow{8}{*}{Visual Finetuning}  & 52.2&68.9 &52.1 &81.3 &  ECCV'24 \\
GLIP-T (A) ~\cite{li2022grounded}   &  & 46.4 &68.7 & 52.7& 84.3 &  CVPR'22 \\
GLIP-T (B) ~\cite{li2022grounded}   &  & 46.6 &70.1 &54.4 & 83.5 &  CVPR'22 \\
RegionClip (Res50) ~\cite{zhong2022regionclip}  &  & 33.9 & 42.3 & 49.4 & 72.6 &  CVPR'22 \\
YOLO-World (Large) ~\cite{cheng2024yolo} & & 47.5 & 69.1 &  54.8 & 81.7 &     CVPR'24 \\
OVDINO (B) ~\cite{wang2024ov}   &   & 52.3 &78.0 & 75.1& 82.1 & ECCV'22 \\
PB-OVD ~\cite{gao2022open}   &   & 26.2 & 40.7&  41.5 & 76.5  & ECCV'22 \\
\hline
GroundingDino (swin-T) ~\cite{liu2023grounding} &  \multirow{5}{*}{Text Prompt}  &34.0 &79.4 &77.9  &80.7 &  ECCV'24 \\
GLIP-T (A) ~\cite{li2022grounded}   &  & 32.6 &71.8 &71.2 & 82.1 &  CVPR'22 \\
GLIP-T (B) ~\cite{li2022grounded}   &  & 27.6 &73.3 &73.2 & 80.6 &  CVPR'22 \\
RegionClip (Res50) ~\cite{zhong2022regionclip}  &  & 17.4 & 7.0 & 6.7 & 8.2 &  CVPR'22 \\
YOLO-World (Large) ~\cite{cheng2024yolo} & & 33.4 & 74.1 & 74.1  & 81.1 &     CVPR'24 \\
OVDINO (B) ~\cite{wang2024ov}   &  &47.1&76.4&61.3&79.9& ECCV'22 \\
PB-OVD ~\cite{gao2022open}   &  & 9.8 &  21.3 &  21.3 & 39.9  & ECCV'22 \\
\hline
\end{tabular}
}
\end{table*}


==> tables/voc2clipart.tex <==
% \begin{table*}[htbp]
%     \centering
%     \caption{Results (\%) on VOC$ \rightarrow $Clipart.}
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c|c|cccccccccccccccccccc|c|c}
%         \hline
%         Method & Finetuning Ways & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & hrs & bike & prsn & plt & sheep & sofa & train & tv & AP\textsubscript{50} & Reference \\
%         \hline
%         GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{7}{*}{Zero Prediction} & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'24   \\
%          GroundingDino (swin-L) ~\cite{liu2023grounding} & & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'24   \\
%         GLIP-T (A) ~\cite{li2022grounded} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22   \\
%         GLIP-T (B) ~\cite{li2022grounded} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22   \\
%         GLIP-T (C) ~\cite{li2022grounded} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22   \\
%         RegionClip (Res50) ~\cite{zhong2022regionclip} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 &  CVPR'22   \\
%         RegionClip (Res50 $\times$ 4) ~\cite{zhong2022regionclip} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 &  CVPR'22   \\
%         OWL-ViT ~\cite{minderer2022simple} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & Arxiv'22  \\
%         OWLv2 ~\cite{minderer2024scaling} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & NeurIPS'24  \\
%         YOLO-World (Large) ~\cite{cheng2024yolo} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'24  \\
%         YOLO-World (Mid) ~\cite{cheng2024yolo} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'24  \\
%         PB-OVD ~\cite{gao2022open} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'22  \\
%         \hline
%          GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{4}{*}{Visual Finetuning}  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'24  \\
%         GLIP-T (A) ~\cite{li2022grounded}&  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 &  CVPR'22   \\
%          GLIP-T (B) ~\cite{li2022grounded}&  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 &  CVPR'22   \\
%         RegionClip (Res50) ~\cite{zhong2022regionclip} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22  \\
%         YOLO-World (Large) ~\cite{cheng2024yolo} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'24  \\
%         PB-OVD ~\cite{gao2022open} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'22  \\
%         \hline
%        GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{3}{*}{Text Prompt}  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'24  \\
%        GLIP-T (A) ~\cite{li2022grounded} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22   \\
%        GLIP-T (B) ~\cite{li2022grounded} &   & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'22   \\
%        YOLO-World (Large) ~\cite{cheng2024yolo} &  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & CVPR'24   \\
%        PB-OVD ~\cite{gao2022open} ~\cite{cheng2024yolo} &  & 26.2 & 48.5 & 32.6 & 33.7 & 38.5 & 54.3 & 37.1 & 18.6 & 34.8 & 58.3 & 12.5 & 12.5 & 33.8 & 65.5 & 54.5 & 52.0 & 9.3 & 24.9 & 54.1 & 49.1 & 38.1 & ECCV'22   \\
%        \hline
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[htbp]
    \centering
    \caption{Results (\%) on VOC$ \rightarrow $Clipart.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|cccccccccccccccccccc|c|c}
        \hline
        Method & Finetuning Ways & aero & bike & bird & boat & bottle & bus & car & cat & chair & cow & table & dog & hrs & bike & prsn & plt & sheep & sofa & train & tv & AP\textsubscript{50} & Reference \\
        \hline
        GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{12}{*}{Zero Prediction} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & ECCV'24   \\
         GroundingDino (swin-L) ~\cite{liu2023grounding} & &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &ECCV'24   \\
        GLIP-T (A) ~\cite{li2022grounded} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & & CVPR'22   \\
        GLIP-T (B) ~\cite{li2022grounded} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
        GLIP-T (C) ~\cite{li2022grounded} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
        RegionClip (Res50) ~\cite{zhong2022regionclip} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
        RegionClip (Res50 $\times$ 4) ~\cite{zhong2022regionclip} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
        OVDINO (A) ~\cite{wang2024ov} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &Arxiv'22  \\
        OVDINO (B) ~\cite{wang2024ov} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &NeurIPS'24  \\
        YOLO-World (Large) ~\cite{cheng2024yolo} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'24  \\
        YOLO-World (Mid) ~\cite{cheng2024yolo} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'24  \\
        PB-OVD ~\cite{gao2022open} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &ECCV'22  \\
        \hline
         GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{6}{*}{Visual Finetuning}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & ECCV'24  \\
        GLIP-T (A) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
         GLIP-T (B) ~\cite{li2022grounded}&  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22   \\
        RegionClip (Res50) ~\cite{zhong2022regionclip} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'22  \\
        YOLO-World (Large) ~\cite{cheng2024yolo} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'24  \\
        PB-OVD ~\cite{gao2022open} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &ECCV'22  \\
        \hline
       GroundingDino (swin-B) ~\cite{liu2023grounding} & \multirow{5}{*}{Text Prompt}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &ECCV'24  \\
       GLIP-T (A) ~\cite{li2022grounded} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & CVPR'22   \\
       GLIP-T (B) ~\cite{li2022grounded} &   &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & CVPR'22   \\
       YOLO-World (Large) ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &CVPR'24   \\
       PB-OVD ~\cite{gao2022open} ~\cite{cheng2024yolo} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &ECCV'22   \\
       \hline
    \end{tabular}
    }
\end{table*}


==> tables/voc2clipartandcomic.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison results (\%) on Pascal VOC→Watercolor (left) and Pascal VOC→Comic (right) with ResNet101 backbone.
For finetune, models are trained on the Pascal VOC, and tested on Watercolor and Comic datasets.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|cccccc|cccccc|l}
\hline
\multirow{2}{*}{Method}&  \multirow{2}{*}{Finetuning Ways} & \multicolumn{6}{c|}{Pascal VOC→Watercolor} & \multicolumn{6}{c|}{Pascal VOC→Comic} & \multirow{2}{*}{Reference} \\ \cline{3-14} 
 &  & bird & car & cat & dog & prsn & AP$_{50}$  & bird & car & cat & dog & prsn & AP$_{50}$ \\ 
 \hline
GroundingDino (swin-T) ~\cite{liu2023grounding} & \multirow{12}{*}{Zero Prediction}& 54.2 &44.5  & 44.5  & 38.8 & 75.8 & 51.6 &28.9 &54.8 &30.7  & 49.1 & 77.1 & 57.7& ECCV'24\\
GroundingDino (swin-B) ~\cite{liu2023grounding}  &  &70.4 &44.3   & 60.4 & 63.5 & 83.8  &64.5 & 59.3 & 68.4 & 43.9 &64.2 &80.8 & 63.3 &ECCV'24\\
GLIP-T (A) ~\cite{li2022grounded} &  & 44.8 & 48.0 &  20.1 & 12.7 & 69.1 & 38.9 & 20.3& 43.0& 7.3 & 14.7 & 66.3 & 30.3 & CVPR'22\\
GLIP-T (B) ~\cite{li2022grounded} &  & 52.1 & 45.8 &  19.1 & 14.6 & 68.4 & 40.0 & 25.6& 51.1& 11.9 & 19.2 & 66.1 & 34.8 & CVPR'22\\
GLIP-T (C) ~\cite{li2022grounded} & & 50.8 & 54.3 & 23.3  & 13.7 & 71.5 & 42.7 &24.4 &51.8 & 10.5 & 14.4 & 66.6 & 33.5& CVPR'22\\
RegionClip (Res50) ~\cite{zhong2022regionclip} & & 17.5 & 23.5 & 20.9 & 11.1 & 29.6 & 24.3 & 16.1 & 27.2 & 18.0 & 20.6 & 26.3 & 21.6 & CVPR'22\\
RegionClip (Res50 $\times$ 4) ~\cite{zhong2022regionclip} &  & 36.0 & 25.3 &  29.7 & 25.2 & 24.5 & 28.1  & 23.4& 25.8& 33.7 & 39.0 & 19.3 & 28.2& CVPR'22\\
OVDINO (A) ~\cite{wang2024ov} &  &46.1&41.5&30.3&25.6&65.5&41.8&17.4&50.5&14.2&11.3&60.2&30.7& Arxiv'22 \\ 
OVDINO (B) ~\cite{wang2024ov} & &48.0&41.4&25.8&30.5&62.7&41.7&21.9&43.6&18.3&14.1&56.1&30.8& NeurIPS'24 \\
YOLO-World (Large) ~\cite{cheng2024yolo} & & 55.2 &47.9 &  34.1 &0.25.8  & 78.3 & 48.3 & 17.7 & 52.3&14.7   & 17.5 & 68.3 &  34.1 & CVPR'24 \\ 
YOLO-World (Mid) ~\cite{cheng2024yolo} & &52.5 &51.4 &32.8 &27.0 &76.7 &48.1 &18.4 &52.1 &12.1 &18.3 &66.7  &33.5   & CVPR'24 \\
PB-OVD ~\cite{gao2022open} & &36.9  & 29.2 & 26.3  & 26.2 &39.1  & 31.5 &19.5 &25.9 &17.2  &22.7  &18.8  & 20.8 & ECCV'22 \\
\hline
GroundingDino (swin-T) ~\cite{liu2023grounding} & \multirow{6}{*}{Visual Finetuning}& 68.6 & 56.7 & 52.3  & 43.4 & 74.2 & 59.0 & 41.4 & 63.6 & 35.4  & 45.0 & 73.6 & 51.8 & ECCV'24\\
GLIP-T (A) ~\cite{li2022grounded} & & 49.8 & 54.3 &  16.4 & 3.5 & 52.5 & 35.3 &7.4 &29.9 & 5.5 & 6.2 & 35.2 &  16.8 & CVPR'22\\
GLIP-T (B) ~\cite{li2022grounded} & & 47.4 & 60.0 &  20.6 & 4.4 & 36.4 & 33.7 & 10.2& 39.9& 7.2 & 6.2 & 16.8 &  16.1 & CVPR'22\\
RegionClip (Res50) ~\cite{zhong2022regionclip} & &  45.4 & 44.3 & 40.2 & 16.7 & 60.8 & 41.5 & 25.2 & 33.9 & 39.7  & 33.2 & 55.9 & 37.6  & CVPR'22\\
YOLO-World (Large) ~\cite{cheng2024yolo} & & 58.0 & 50.7  & 373. & 22.0  & 75.7  &48.7 &19.2 &54.7 & 11.8 & 15.5 & 61.1 & 32.5 & CVPR'24\\ 
YOLO-World (Medium) ~\cite{cheng2024yolo} & &33.0  & 29.7 &19.2   &17.2  &43.6  &28.5  &12.8 &34.8 &7.0  &9.5  &31.6  &19.1   & CVPR'24\\ 
OVDINO (B) ~\cite{wang2024ov} & &56.6&57.9&26.8&23.8&70.3&47.1&20.7&44.8&19.7&13.9&57.9&31.4& ECCV'22\\
PB-OVD ~\cite{gao2022open} & & 48.2&  43.3& 28.0 & 18.5 &  57.7& 39.1 & 16.5 & 22.9 &  18.5 & 13.0 & 36.0 & 21.4 & ECCV'22\\
\hline
GroundingDino (swin-T) ~\cite{liu2023grounding} & \multirow{5}{*}{Text Prompt}& 59.9 & 49.2 & 46.4  & 50.0 & 80.7 & 57.2 &39.3 &61.1 & 43.3 & 59.5 & 79.2 &56.5 & ECCV'24\\
GLIP-T (A) ~\cite{li2022grounded} & & 45.6 & 48.9 & 21.7  & 14 & 69.8 & 40.0 &19.6 &43.5 & 7.1 & 14.3 & 65.7 & 30.0 & CVPR'22\\
GLIP-T (B) ~\cite{li2022grounded} & & 52.1 & 44.5 &  19.4 & 14.8 & 68.4 & 39.8 & 24.8&50.2 & 11.6 & 19.3 & 66 & 34.4 & CVPR'22\\
YOLO-World (Large) ~\cite{cheng2024yolo} & & 54.4 & 45.3 & 28.9  & 18.7 & 73.0 & 44.1 & 13.9 & 53.9 & 12.1 & 14.0 & 64.8 & 31.7 & CVPR'24\\ 
OVDINO (B) ~\cite{wang2024ov} & &46.7&38.7&26.5&32.1&64.8&41.8&20.4&45.4&17.9&14.4&57.4&31.1& ECCV'22\\
PB-OVD ~\cite{gao2022open} & & 36.1 & 34.7 & 22.5  & 13.3 & 48.2 & 31.0 & 6.4& 15.6 & 5.3 & 9.3 & 18.2 & 11.0& ECCV'22\\
\hline
\end{tabular}
}
\end{table*}

==> tables/voc2clipartandcomic_second.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison results (\%) on Pascal VOC→Watercolor (left) and Pascal VOC→Comic (right) with ResNet101 backbone.
For finetune, models are trained on the Pascal VOC, and tested on Watercolor and Comic datasets.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|ccccccc|ccccccc|l}
\hline
\multirow{2}{*}{Method}&  \multirow{2}{*}{Finetuning Ways} & \multicolumn{7}{c|}{Pascal VOC→Watercolor} & \multicolumn{7}{c|}{Pascal VOC→Comic} & \multirow{2}{*}{Reference} \\ \cline{3-16} 
 & & bike & bird & car & cat & dog & prsn & AP$_{50}$  & bike & bird & car & cat & dog & prsn & AP$_{50}$ \\ 
 \hline
OADP ~\cite{wang2023object} & \multirow{10}{*}{Visual finetuning}&   &  &  &   &  &  &  &  & & &  &  &  & & ECCV'24\\
BARON ~\cite{wu2023aligning}  & &   &  &  &   &  &  &  &  & & &  &  &  &  & ECCV'24\\
VL-PLM ~\cite{zhao2022exploiting} & &   &  &  &   &  &  &  &  & & &  &  &  &  & CVPR'22\\
DST-Det ~\cite{xu2023dst} & &   &  &  &   &  &  &  &  & & &  &  &  &  & CVPR'22\\
PromptDet ~\cite{feng2022promptdet} & &   &  &  &   &  &  &  &  & & &  &  &  & & CVPR'22\\
DetPro\cite{du2022learning} & &   &  &  &  &  &  &  &  &  &  &  &  &  &  & CVPR'22\\
Detic ~\cite{zhou2022detecting} & &   &  &  &   &  &  &  &  & & &  &  &  & & CVPR'22\\
OpenSeeD~\cite{zhang2023simple} & &   &  &  &   &  &  &  &  & & &  &  &  &  & Arxiv'22 \\ 
mm-ovod ~\cite{kaul2023multi} & &   &  &  &   &  &  &  &  & & &  &  &  &  & NeurIPS'24 \\
LAMI-DETR ~\cite{du2025lami} & &   &  & &   &  &  &  &  &  & &   &  &  &   & CVPR'24 \\ 
\hline
\end{tabular}
}
\end{table*}
